Can visual language models resolve textual ambiguity with visual cues? Let visual puns tell you!

Humans possess multimodal literacy, allowing them to actively integrate information from various modalities to form reasoning. Faced with challenges like lexical ambiguity in text, we supplement this with other modalities, such as thumbnail images or textbook illustrations. Is it possible for machines to achieve a similar multimodal understanding capability? In response, we present Understanding Pun with Image Explanations (UNPIE), a novel benchmark designed to assess the impact of multimodal inputs in resolving lexical ambiguities. Puns serve as the ideal subject for this evaluation due to their intrinsic ambiguity. Our dataset includes 1,000 puns, each accompanied by an image that explains both meanings. We pose three multimodal challenges with the annotations to assess different aspects of multimodal literacy; Pun Grounding, Disambiguation, and Reconstruction. The results indicate that various Socratic Models and Visual-Language Models improve over the text-only models when given visual context, particularly as the complexity of the tasks increases.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/3_vlm_mmt.tex <==
\section{Are VLMs for MMT?}
\label{sec:vlm_mmt}

Multimodal Machine Translation (MMT) is a translation task that typically provides an image as context in addition to the text in the source language.
Previous approaches~\cite{} to MMT design task-specific architectures and optimize them on training datasets with multimodal annotation such as Multi30k~\cite{}.
In this section, we challenge \textit{whether such task-specific design is necessary for MMT} using general-purpose visual-language models (VLMs).
VLMs (\eg Flamingo~\cite{}, LLaVA~\cite{}, and LLAMA-Adapter~\cite{}) are general-purpose instruction followers that can output suitable responses to diverse queries from \textit{Who drew this picture?} to \textit{What are the things I should be cautious about when I visit here?}.
We first apply a VLM directly to a popular MMT benchmark.
\jw{TODO: complete rewrite}

\input{tabs/en-fr_results}

\subsection{VLMs Outperform Task-Specific Designs}
\label{subsec:vlms_outperform}

\textbf{Dataset}.
Multi30k~\cite{} is a widely used dataset for MMT tasks.
It extends Flickr30k~\cite{} and MSCOCO~\cite{} image captioning datasets to German and French caption targets.
The dataset offers a single Train set, a Validation set, and three test sets (Test2016, Test2017, and MSCOCO).
We train and evaluate data on the pre-defined splits of Multi30k following previous literature~\cite{}.

\textbf{Models}.
As an instance of general-purpose VLM, we adopt the visual instruction tuning model LLaVA-1.5.
LLaVA~\cite{} is a general-purpose visual and language understanding model built on top of the large language model Vicuna~\cite{}.
LLaVA-1.5~\cite{} extends LLaVA with a larger image encoder (CLIP-ViT-L-336px~\cite{}) and additional VQA data to achieve state-of-the-art among 11 benchmarks.
We use Low-Rank Adaptation (LoRA)~\cite{} to transfer LLaVA to Multi30k with minimum additional resources. Please refer to~\cref{sec:appendix_hyperparams} for the training details.
We also adopt various baselines that do or do not require the visual context at inference time: refer to~\cref{sec:related_Work} for their details.

\textbf{Results}.
Table~\ref{tab:main_table_fr} summarizes how the general-purpose VLM performs compared to the state-of-the-art architectures on Multi30k.
Zeroshot LLaVA performs reasonably and shows that it has translation capability, albeit being outmatched by most of the baselines.
However, further fine-tuning the VLM with LoRA is necessary for it to surpass all the baselines without any architectural modification.
We conclude that similarly to other multimodal tasks, Multimodal Machine Translation can be tackled better with pre-trained multimodal knowledge in VLMs than with complex model architectures specifically designed for the task.
Still, task-specific fine-tuning is necessary for better translation quality.

\subsection{Fine-Tuning Undermines Visual Specificity}
\label{subsec:ft_bad}

However, this evaluation on the Multi30k dataset tells only one side of the story.
The other side is that Multi30k may not be a reliable testbed for ambiguity modeling.
After all, results in Table~\ref{tab:main_table_fr} show that the visual context (V + L) only offers a marginal improvement over the text-only translation (L) both in zero-shot and fine-tuned VLMs.
While a previous study reported that there is a negative correlation between
lexical ambiguity and translation quality in Multi30k~\cite{},
yet another reported that there are not so many ambiguous samples in the dataset in the first place~\cite{}. In fact, only $~2\%$ of each test set in Multi30k required such ambiguity modeling upon manual inspection~\cite{}.
Hence, we employ another benchmark with a focus on the ambiguity resolution problem.

\textbf{Dataset}.
Contrastive Multilingual Multimodal Translation Evaluation (CoMMuTE) dataset~\cite{}
provides a closer look at the ambiguity problem. It builds on 155 ambiguous English sentences and asks the machines to translate them into German, French, or Czech.
Each sentence has a single ambiguous word in it along with two different image contexts describing different meanings of the word.

\textbf{Metrics}.
CoMMuTE is formulated as a binary classification task of deciding which translation
is better aligned with the given image context.
A model that assigns a higher score to the correct image-translation pair gets a higher accuracy.
The original paper uses the perplexity (PPL) of the sentence as the goodness score: $PPL_p(y|x,v) = \prod_{i=1}^N p(y_i|y_{<i},x,v)^{1/N}$, where $y_i$ is each token of the translated target $y$, $x$ is the source text sequence, $v$ is the visual context, and $p(y_i|y_{<i},x,v)$ is the autoregressive next-token likelihood given by the model.

However, perplexity might not correctly represent how well the model-generated text would reflect the visual context.
When both of the considered target candidates have low likelihood and thus large perplexities as measured by the model, the generated text would contain neither
of the candidates.
Hence, we also report the generation score (GEN).
We first generate a translation hypothesis using the model. 
Then, we compute the distance between the hypothesis and each target candidate
to select the candidate most similar to the generated text.
We use BERTScore~\cite{} as the text distance metric.

\input{tabs/commute}

\textbf{Results}.
Table~\ref{tab:commute} shows that both our zero-shot and LoRA-finetuned VLM models can better discriminate ambiguous translation targets than all the baselines, including VGAMT which was proposed alongside the benchmark as a resolution.
However, the task-specific fine-tuning process on Multi30k actually degrades the visual alignment accuracy in CoMMuTE (LLaVA-Zeroshot vs. LLaVA-LoRA) as measured by the original perplexity score (PPL).
While the fine-tuned model saw an increase in GEN-based accuracy for translation to French, this came at an immense loss of the PPL-based accuracy.
We observed that LLaVA without fine-tuning often generates text
different in style from both of the translation targets, which is unfavorable for generation-based scoring (GEN). 

==> sec/3_vlm_mmt_backup.tex <==
\section{Are VLMs for MMT?}
\label{sec:vlm_mmt}

Multimodal Machine Translation (MMT) is a translation task that typically provides an image as context in addition to the text in the source language.
Previous approaches~\cite{} to MMT design task-specific architectures and optimize them on training datasets with multimodal annotation such as Multi30k~\cite{}.
In this section, we challenge \textit{whether such task-specific design is necessary for MMT} using general-purpose visual-language models (VLMs).
VLMs (\eg Flamingo~\cite{}, LLaVA~\cite{}, and LLAMA-Adapter~\cite{}) are general-purpose instruction followers that can output suitable responses to diverse queries from \textit{Who drew this picture?} to \textit{What are the things I should be cautious about when I visit here?}.
We first apply a VLM directly to a popular MMT benchmark.
\jw{TODO: complete rewrite}

\input{tabs/en-fr_results}

\subsection{VLMs Outperform Task-Specific Designs}
\label{subsec:vlms_outperform}

\textbf{Dataset}.
Multi30k~\cite{} is a widely used dataset for MMT tasks.
It extends Flickr30k~\cite{} and MSCOCO~\cite{} image captioning datasets to German and French caption targets.
The dataset offers a single Train set, a Validation set, and three test sets (Test2016, Test2017, and MSCOCO).
We train and evaluate data on the pre-defined splits of Multi30k following previous literature~\cite{}.

\textbf{Models}.
As an instance of general-purpose VLM, we adopt the visual instruction tuning model LLaVA-1.5.
LLaVA~\cite{} is a general-purpose visual and language understanding model built on top of the large language model Vicuna~\cite{}.
LLaVA-1.5~\cite{} extends LLaVA with a larger image encoder (CLIP-ViT-L-336px~\cite{}) and additional VQA data to achieve state-of-the-art among 11 benchmarks.
We use Low-Rank Adaptation (LoRA)~\cite{} to transfer LLaVA to Multi30k with minimum additional resources. Please refer to~\cref{sec:appendix_hyperparams} for the training details.
We also adopt various baselines that do or do not require the visual context at inference time: refer to~\cref{sec:related_Work} for their details.

\textbf{Results}.
Table~\ref{tab:main_table_fr} summarizes how the general-purpose VLM performs compared to the state-of-the-art architectures on Multi30k.
Zeroshot LLaVA performs reasonably and shows that it has translation capability, albeit being outmatched by most of the baselines.
However, further fine-tuning the VLM with LoRA is necessary for it to surpass all the baselines without any architectural modification.
We conclude that similarly to other multimodal tasks, Multimodal Machine Translation can be tackled better with pre-trained multimodal knowledge in VLMs than with complex model architectures specifically designed for the task.
Still, task-specific fine-tuning is necessary for better translation quality.

\subsection{Fine-Tuning Undermines Visual Specificity}
\label{subsec:ft_bad}

However, this evaluation on the Multi30k dataset tells only one side of the story.
The other side is that Multi30k may not be a reliable testbed for ambiguity modeling.
After all, results in Table~\ref{tab:main_table_fr} show that the visual context (V + L) only offers a marginal improvement over the text-only translation (L) both in zero-shot and fine-tuned VLMs.
While a previous study reported that there is a negative correlation between
lexical ambiguity and translation quality in Multi30k~\cite{},
yet another reported that there are not so many ambiguous samples in the dataset in the first place~\cite{}. In fact, only $~2\%$ of each test set in Multi30k required such ambiguity modeling upon manual inspection~\cite{}.
Hence, we employ another benchmark with a focus on the ambiguity resolution problem.

\textbf{Dataset}.
Contrastive Multilingual Multimodal Translation Evaluation (CoMMuTE) dataset~\cite{}
provides a closer look at the ambiguity problem. It builds on 155 ambiguous English sentences and asks the machines to translate them into German, French, or Czech.
Each sentence has a single ambiguous word in it along with two different image contexts describing different meanings of the word.

\textbf{Metrics}.
CoMMuTE is formulated as a binary classification task of deciding which translation
is better aligned with the given image context.
A model that assigns a higher score to the correct image-translation pair gets a higher accuracy.
The original paper uses the perplexity (PPL) of the sentence as the goodness score: $PPL_p(y|x,v) = \prod_{i=1}^N p(y_i|y_{<i},x,v)^{1/N}$, where $y_i$ is each token of the translated target $y$, $x$ is the source text sequence, $v$ is the visual context, and $p(y_i|y_{<i},x,v)$ is the autoregressive next-token likelihood given by the model.

However, perplexity might not correctly represent how well the model-generated text would reflect the visual context.
When both of the considered target candidates have low likelihood and thus large perplexities as measured by the model, the generated text would contain neither
of the candidates.
Hence, we also report the generation score (GEN).
We first generate a translation hypothesis using the model. 
Then, we compute the distance between the hypothesis and each target candidate
to select the candidate most similar to the generated text.
We use BERTScore~\cite{} as the text distance metric.

\input{tabs/commute}

\textbf{Results}.
Table~\ref{tab:commute} shows that both our zero-shot and LoRA-finetuned VLM models can better discriminate ambiguous translation targets than all the baselines, including VGAMT which was proposed alongside the benchmark as a resolution.
However, the task-specific fine-tuning process on Multi30k actually degrades the visual alignment accuracy in CoMMuTE (LLaVA-Zeroshot vs. LLaVA-LoRA) as measured by the original perplexity score (PPL).
While the fine-tuned model saw an increase in GEN-based accuracy for translation to French, this came at an immense loss of the PPL-based accuracy.
We observed that LLaVA without fine-tuning often generates text
different in style from both of the translation targets, which is unfavorable for generation-based scoring (GEN). 

==> sec/ax_4_fine_grained_results.tex <==
\section{Fine-Grained Results}
\label{sec:appendix_fine_grained_results}

% \input{tabs/ax_pbj_recon}
\input{tabs/ax_pun_reconstruction}

% \input{tabs/ax_task1}

% \input{tabs/ax_task2}

==> tabs/ax_pbj_recon.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{
    \centering\small
    \begin{tabular}{lcccccccccc} \toprule
    \multicolumn{11}{c}{\bf De$\rightarrow$En} \\\midrule 
    & & \multicolumn{3}{c}{All} & \multicolumn{3}{c}{Hetero} & \multicolumn{3}{c}{Homo} \\ 
    Model & Modalities & Correctness & Bleu-4 & Meteor & Correctness & Bleu-4 & Meteor & Correctness & Bleu-4 & Meteor \\
    \midrule
    LLAVA-Zeroshot & L & & & & & & & & \\
    LLAVA-Zeroshot & V + L & & & & & & & & \\
    LLAVA-LoRA & L & & & & & & & & \\
    LLAVA-LoRA & V + L & & & & & & & & \\
    \midrule
    Vicuna & L & 32.45 & - & - & 23.9 & - & - & 41.0 & - & - \\
    Vicuna + BLIP-2 & V + L & 33.65 & - & - & 23.0 & - & - & 44.3 & - & -\\
    GPT4 & L & 64.95 & 43.61 & 0.75 & 55.1 & 41.59 & 0.74 &74.8 & 45.945 & 0.75\\
    GPT4 + BLIP-2 & V + L & 68.45 & 41.37 & 0.73 & 59.6&38.21 &0.70 & 77.3 &43.545 & 0.735 \\
    %GPT4V(ision) & V + L & 67.25&29.3 & 0.63& 59.5& 29.22& 0.62&75.0 &29.4 & 0.645 \\
    \midrule
    \midrule
    \multicolumn{11}{c}{\bf Fr$\rightarrow$En} \\\midrule 
    LLAVA-Zeroshot & L & & & & & & & & \\
    LLAVA-Zeroshot & V + L & & & & & & & & \\
    LLAVA-LoRA & L & & & & & & & & \\
    LLAVA-LoRA & V + L & & & & & & & & \\
    \midrule
    Vicuna & L & 36.55 & - & - & 26.7 & - & - & 46.4 & - & - \\
    Vicuna + BLIP-2 & V + L & 36.0 & - & - & 25.0 & - & - & 47.0 & - & -\\
    GPT4 & L & 63.65& 43.15& 0.74& 53.6& 41.78 & 0.74 & 73.7 & 44.715 & 0.735\\
    GPT4 + BLIP-2 & V + L & 66.0 & 39.75 & 0.71 & 55.1 & 38.21 & 0.7 & 76.9 &  41.48&0.72\\
    %GPT4V(ision) & V + L & 64.0& 29.53 &0.63 &55.0 &29.9 & 0.62&73.0 &29.145 &0.635\\
    \midrule
    \midrule
    \multicolumn{11}{c}{\bf Ko$\rightarrow$En} \\\midrule 
    LLAVA-Zeroshot & L & & & & & & & & \\
    LLAVA-Zeroshot & V + L & & & & & & & & \\
    LLAVA-LoRA & L & & & & & & & & \\
    LLAVA-LoRA & V + L & & & & & & & & \\
    \midrule
    Vicuna & L & 17.95 & - & - & 8.9 & - & - & 27.0 & - & - \\
    Vicuna + BLIP-2 & V + L & 20.1 & - & - & 12.0 & - & - & 28.2 & - & -\\
    
    GPT4 & L &54.0 &28.03 & 0.63 & 44.6& 26.43& 0.62&63.4& 29.855& 0.63\\
    GPT4 + BLIP-2 & V + L & 56.6& 25.18& 0.6& 47.0& 23.89& 0.59& 66.2& 26.625 & 0.61 \\
    % GPT4V(ision) & V + L & 61.75& 17.83 & 0.57 &50.0 & 16.02 & 0.56 &73.5 &19.63 & 0.57\\
    \bottomrule
    
    \end{tabular}
    }
    %\vspace{-.2cm}
    \caption{Pun Reconstruction Full table}%\vspace{-.3cm}}
    \label{tab:ax_pbj_recon}
\end{table*}
 

==> tabs/ax_pun_reconstruction.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{
    \centering\small
    \begin{tabular}{llcccccccccc} \toprule
    \multicolumn{12}{c}{\bf De$\rightarrow$En} \\\midrule 
    & & & \multicolumn{3}{c}{Hetero} & \multicolumn{3}{c}{Homo} & \multicolumn{3}{c}{All} \\ 
    & Model & Inputs & Correct (\%) & Bleu-4 & METEOR & Correct (\%) & Bleu-4 & METEOR & Correct (\%) & Bleu-4 & METEOR \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LM}}}
    & Vicuna & L & 23.9 &28.4 &61.2 & 41.0 & 28.3& 61.5& 32.5&28.3&61.3\\
    & GPT-4 & L & 55.1 &41.6 & 73.5& 74.8 &45.9 &75.0 & 65.0 &43.6&74.3\\
    & Qwen-VL-C & L & 25.2 & 30.6 & 67.4 & 31.5 & 14.9 & 51.1 & 28.4 & 22.4 & 59.3 \\
    & LLAVA & L & 36.0  & 35.9  & 67.3 & 37.8 & 15.5 & 51.2 & 36.9 & 24.5 & 59.2 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 23.0 & 21.2& 54.2& 44.3 &21.7 &54.7 & 33.7&21.4& 54.4 \\
    & GPT-4 & V + L & 59.6 & 39.5 & 71.5& 77.3 & 43.5&73.9 & 68.5 &41.4&72.8\\
    \midrule
    \parbox[t]{1.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL-C & V + L & 36.0 & 38.1 & 68.7 & 36.9 & 16.7 & 52.3 & 36.5 & 26.1 & 68.7 \\
    & LLAVA & V + L & 38.7 & 37.5 & 68.3 & 42.3 & 13.7 & 53.9 & 40.5 & 26.2 & 61.1 \\
    & LLAVA-MMT & V + L & 31.5 & 25.6 & 45.7 & 27.0 & 12.3 & 38.1 & 29.3 & 18.5 & 41.9 \\
    \midrule
    \midrule
    \multicolumn{12}{c}{\bf Fr$\rightarrow$En} \\\midrule 
    \parbox[t]{1.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LM}}}
    & Vicuna & L & 26.7 & 32.1 & 63.6 & 46.4 & 33.5&64.8 & 36.6 &32.8& 64.2  \\
    & GPT-4 & L & 53.6 & 41.8 & 74.0& 73.7 & 44.7& 73.4& 63.7 & 43.1& 73.6\\
    & Qwen-VL-C & L & 31.5 & 30.3 & 66.3 & 36.0 & 15.5 & 51.2 & 33.8 & 22.6 & 58.8 \\
    & LLAVA & L & 40.5 & 39.3 & 70.0 & 36.9 & 17.3 & 53.6 & 38.7 & 26.9 & 61.8 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 25.0 & 26.3& 57.8& 47.0 & 25.6& 58.3& 36.0 &25.9&58.1\\
    & GPT-4 & V + L & 55.1 & 38.2& 70.0& 76.9 & 41.5&71.9 & 66.0 & 39.8 &71.0 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL-C & V + L & 39.6 & 25.7 & 59.8 & 38.7 & 16.8 & 52.0 & 39.2 & 15.5 & 51.2 \\
    & LLAVA & V + L & 36.0 & 38.2 & 68.0 & 41.4 & 18.5 & 54.2 & 38.7 & 27.2 & 61.1 \\
    & LLAVA-MMT & V + L & 27.0 & 24.3 & 43.2 & 33.3 & 12.9 & 39.3 & 30.2 & 17.8 & 41.3  \\
    \midrule
    \midrule
    \multicolumn{12}{c}{\bf Ko$\rightarrow$En} \\\midrule 
    \parbox[t]{1.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LM}}}
    & Vicuna & L & 8.9 &12.4 &43.6 & 27.0 & 13.7&44.7 & 18.0 &13.1&44.1\\
    & GPT-4 & L & 44.6 &26.4 &62.0 & 63.4 &29.9 &63.1 & 54.0 & 28.0& 62.7\\
    & Qwen-VL-C & L & 13.5 & 12.9 & 47.2 & 25.2 & 7.3 & 38.2 & 19.4 & 10.0 & 42.7 \\
    & LLAVA & L & 22.5 & 19.2 & 49.0 & 27.9 & 10.7 & 41.9 & 25.2 & 14.4 & 45.5 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 12.0 & 7.8&37.4 & 28.2 & 8.9&39.0 & 20.1 &8.3&38.2\\
    & GPT-4 & V + L & 47.0 & 23.9& 59.0& 66.2 &26.6 & 60.9& 56.6 & 25.2&60.0 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL-C & V + L & 21.6 & 16.3 & 47.9 & 31.5 & 8.6 & 39.7 & 26.6 & 12.0 & 43.8 \\
    & LLAVA & V + L & 25.2 & 17.8 & 49.1 & 41.4 & 10.4 & 42.3 & 33.3 & 13.7 & 45.7 \\
    & LLAVA-MMT & V + L &  18.3 & 15.0 & 46.7 & 28.0 & 6.3 & 38.5 & 23.3 & 10.7 & 42.6  \\
    \bottomrule
    \end{tabular}
    }
    %\vspace{-.2cm}
    \caption{Fine-grained results on pun reconstruction task, including Bleu-4 and METEOR scores per each language (Fr and Ko) and category (Hetero and Homo).}%\vsace{-.3cm}}
    \label{tab:ax_pun_reconstruction}
\end{table*}
 

==> tabs/ax_task1.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Pun type & Model& L & V+L  \\
    \midrule
    Homographic&GPT4 & 96.8 & 97.2 \\
    &Vicuna  & 43.8 &  57.8 \\
    Heterographic&GPT4 & 94.2 & 95.0 \\
    &Vicuna  & 50.0 & 61.4  \\
    
    \bottomrule
    \end{tabular}
    \caption{task1}
    \label{tab:ax_task1}
\end{table}

==> tabs/ax_task2.tex <==
\begin{table}[ht]
    \centering\small
    \begin{tabular}{lccc} \toprule
    Model & Language & Homographic & Heterographic  \\
    \midrule
     & De & 68.2 & 74.6 \\
    GPT4+BLIP2 & Fr & 69.0 & 76.8\\
     & Ko & 65.4 & 66.2\\
  
     \midrule
    \midrule
   
    
    \end{tabular}
    
    %\vspace{-.2cm}
    \caption{task2}
    \label{tab:ax_task2}
\end{table}


 

==> tabs/backup_pun_dis.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{l@{\hskip 1.3mm}l@{\hskip 1.3mm}c@{\hskip 1.3mm}ccccccccc}
    \toprule
    &  &  
    & \multicolumn{3}{c}{\bf En $\rightarrow$ De}
    & \multicolumn{3}{c}{\bf En $\rightarrow$ Fr}
    & \multicolumn{3}{c}{\bf En $\rightarrow$ Ko} \\
    & Model & Inputs
    & Homo & Hetero & All
    & Homo & Hetero & All
    & Homo & Hetero & All \\
    \midrule
    & Random & & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\
    \midrule
    \parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 59.4& 64.4& 61.9 &61.4 & \underline{72.2}& 66.8& 55.4& 55.2& 55.3\\
    & GPT-4 & V + L & \textbf{68.2} & \textbf{74.6} & \textbf{71.4} & \textbf{69.0} & 
    \textbf{76.8} & \textbf{72.9} & \textbf{65.4} & \textbf{66.2} & \textbf{65.8} \\
    \midrule
    \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL & V + L & 60.7 & 64.4 & 62.6 & 61.7 & 71.4 & 66.5 & 55.4 & \underline{57.2}& 56.3 \\
    & LLAVA & V + L & \underline{65.1} & \underline{70.8} & \underline{68.0} & 61.1 & 70.6 & 65.8 & \underline{58.1} & 56.9 & \underline{57.5} \\
    & LLAVA-MMT & V + L & 63.5 & 68.0 & 65.7 & \underline{64.1} & 70.0 & \underline{67.0} & 56.6 & 56.1 & 56.4 \\
    \bottomrule
    \end{tabular}
    \caption{Experimental results on the pun disambiguation task. All scores are reported in terms of binary classification accuracy. The best scores are \textbf{bolded} and the second-best ones are \underline{underlined}.}
    \label{tab:pun_disambiguation}
\end{table*}

==> tabs/backup_pun_reconstruction.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{
    \centering
    \begin{tabular}{llcccccccccc} \toprule
    \multicolumn{8}{c}{\bf De$\rightarrow$En} \\\midrule 
    & & & \multicolumn{3}{c}{Hetero} & \multicolumn{3}{c}{Homo} & \multicolumn{3}{c}{All} \\ 
    & Model & Inputs 
    & Correct (\%) & Bleu-4 & METEOR 
    & Correct (\%) & Bleu-4 & METEOR
    & Correct (\%) & Bleu-4 & METEOR \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LM}}}
    & Vicuna & L & 23.9 & 41.0 & 32.5&28.3&61.3\\
    & GPT-4 & L & 55.1 & 74.8  & 65.0 &43.6&74.3\\
    & Qwen-VL-C & L & 25.2  & 31.5  & 28.4 & 22.4 & 59.3 \\
    & LLAVA & L & 36.0   & 37.8  & 36.9 & 24.5 & 59.2 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 23.0 ($\uparrow$ 0.9) & 44.3 ($\uparrow$ 3.3)& 33.7 ($\uparrow$ 1.2)&21.4 ($\downarrow$ 6.9)& 54.4 ($\downarrow$ 5.9) \\
    & GPT-4 & V + L & 59.6 ($\uparrow$ 4.5)& 77.3 ($\uparrow$ 3.5) & 68.5 ($\uparrow$ 3.5) &41.4 ($\downarrow$ 2.2)&72.8 ($\downarrow$ 1.5)\\
    \midrule
    \parbox[t]{1.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL-C & V + L & 36.0 ($\uparrow$ \textbf{10.8}) & 36.9 ($\uparrow$ \textbf{5.4})& 36.5 ($\uparrow$ \textbf{12.1}) & 26.1 ($\uparrow$ \textbf{3.8}) & 68.7 ($\uparrow$ \textbf{1.8})\\
    & LLAVA & V + L & 38.7 ($\uparrow$ 2.7)& 42.3 ($\uparrow$ 4.5)& 40.5 ($\uparrow$ 3.6)& 26.2 ($\uparrow$ 1.7)& 61.1 ($\uparrow$ \textbf{1.8})\\
    & LLAVA-MMT & V + L & 31.5 & 27.0 & 29.3 & 18.5 & 41.9 \\
    \midrule
    \midrule
    \multicolumn{8}{c}{\bf Ko$\rightarrow$En}
    \\\midrule 
    \parbox[t]{1.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LM}}}
    & Vicuna & L & 26.7  & 46.4 & 36.6 &32.8& 64.2  \\
    & GPT-4 & L & 53.6 & 73.7 & 63.7 & 43.1& 73.6\\
    & Qwen-VL-C & L & 31.5  & 36.0  & 33.8 & 22.6 & 58.8 \\
    & LLAVA & L & 40.5 & 36.9 & 38.7 & 26.9 & 61.8 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 25.0 & 47.0 & 36.0 &25.9&58.1\\
    & GPT-4 & V + L & 55.1 & 76.9 & 66.0 & 39.8 &71.0 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL-C & V + L & 39.6 & 38.7 & 39.2 & 15.5 & 51.2 \\
    & LLAVA & V + L & 36.0 & 41.4 & 38.7 & 27.2 & 61.1 \\
    & LLAVA-MMT & V + L & 27.0 & 33.3 & 30.2 & 17.8 & 41.3  \\
    \midrule
    \midrule
    \multicolumn{8}{c}{\bf Ko$\rightarrow$En} \\\midrule 
    \parbox[t]{1.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LM}}}
    & Vicuna & L & 8.9 & 27.0 & 18.0 &13.1&44.1\\
    & GPT-4 & L & 44.6 & 63.4 & 54.0 & 28.0& 62.7\\
    & Qwen-VL-C & L & 13.5 & 25.2 & 19.4 & 10.0 & 42.7 \\
    & LLAVA & L & 22.5 & 27.9 & 25.2 & 14.4 & 45.5 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{SM}}}
    & Vicuna & V + L & 12.0 & 28.2 & 20.1 &8.3&38.2\\
    & GPT-4 & V + L & 47.0 & 66.2 & 56.6 & 25.2&60.0 \\
    \midrule
    \parbox[t]{1.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{VLM}}}
    & Qwen-VL-C & V + L & 21.6 & 31.5 & 26.6 & 12.0 & 43.8 \\
    & LLAVA & V + L & 25.2 & 41.4 & 33.3 & 13.7 & 45.7 \\
    & LLAVA-MMT & V + L &  18.3 & 28.0 & 23.3 & 10.7 & 42.6  \\
    \bottomrule
    \end{tabular}
    }
    %\vspace{-.2cm}
    \caption{Outcomes for the pun reconstruction task, where $\uparrow$ and $\downarrow$ signify the performance change attributed to the inclusion of visual context.
    The model with the largest performance increase is marked \textbf{bold} in each language.
    % Comprehensive results can be found in Table~\ref{tab:ax_pun_reconstruction} of~\cref{sec:appendix_fine_grained_results}.
    }%\vspace{-.3cm}}
    \label{tab:pun_reconstruction}
\end{table*}
 

==> tabs/commute.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{2}{c}{\bf En$\rightarrow$Fr} & \multicolumn{2}{c}{\bf En$\rightarrow$De} \\
    \midrule
    & \multicolumn{4}{c}{Accuracy} \\
    Model & PPL & GEN & PPL & GEN   \\
    \midrule
    Gated Fusion & 50.0 & - & 49.7 & - \\
    Graph-MMT & 50.2 & - & 49.1 & -  \\
    VGAMT & 67.1 & - & 59.0 & - \\
    LLAVA-Zeroshot & \textbf{89.6} & 64.3 & \textbf{69.0} & \textbf{67.7} \\
    LLAVA-LoRA & 77.6 & \textbf{70.1} & 66.7 & 61.3 \\
    \bottomrule
    \end{tabular}
    \caption{Results in CoMMuTE binary classification dataset. The best scores are \textbf{bolded}.}
    \label{tab:commute}
\end{table}

==> tabs/en-fr_results.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{
    \centering\small
    \begin{tabular}{lcccccccc} \toprule
    \multicolumn{9}{c}{\bf En$\rightarrow$Fr} \\\midrule 
    & & \# trainable & \multicolumn{2}{c}{Test2016} & \multicolumn{2}{c}{Test2017} & \multicolumn{2}{c}{MSCOCO} \\ 
    Model & Modalities & params & BLEU & METEOR & BLEU & METEOR & BLEU & METEOR \\ \midrule
    
    mBART-Finetune~\cite{futeral-etal-2023-tackling} & L & 12.6M & \underline{67.2} & 79.9 &  \underline{61.5} & 76.0 & \textbf{51.5} & 69.5 \\

    VALHALLA~\cite{li2022valhalla} & L & - & 63.1 & 81.8 & 56.0 & 77.1 & 46.5 & 71.4 \\
    
    CLIP-Trans~\cite{gupta2023cliptrans} & L & - & 64.6 & \underline{82.5} & 57.6 & \underline{77.8} & 48.8 & \underline{72.8} \\
    
    CAP-ALL~\cite{li2021feature} & V + L & - & 60.1 & 74.3 & 52.8 & 68.6 & 44.3 & 62.6 \\
    DCCN~\cite{lin2020dynamic} & V + L & - & 61.2 & 76.4 & 54.3 & 70.3 & 45.4 & 65.0 \\
    
    Gated Fusion~\cite{wu2021good} & V + L & 2.8M & 61.7 & 81.0 & 54.8 & 77.1 & 44.9 & 71.4 \\
    
    Graph-MMT~\cite{yin2020novel}
    & V + L  & 4.0M &  58.9 & 74.1 &  51.5 & 68.7  &  41.0  & 61.6  \\
  
    VGAMT~\cite{futeral-etal-2023-tackling} & V + L & 13.2M & \underline{67.2} & 79.7  & \textbf{61.6} & 75.9  & \underline{51.1} & 68.9 \\

    \hline
    LLAVA-Zeroshot & L & - & 41.4 & 69.8 & 38.7 & 66.5 & 41.0 & 67.8 \\
    LLAVA-LoRA & L & 13.1M & 67.1 & 84.4 & 59.6 & 79.4 & 50.0 & 73.6 \\
    LLAVA-Zeroshot & V + L & - & 40.9 & 69.4 & 40.7 & 68.2 & 41.0 & 68.1 \\
    LLAVA-LoRA & V + L & 13.1M & \textbf{68.2} & \textbf{85.0} & 60.8 & \textbf{80.2} & 50.8 & \textbf{74.5} \\
    
    \midrule
    \midrule
    \multicolumn{9}{c}{\bf En$\rightarrow$De} \\\midrule 
    
    mBART-Finetune~\cite{futeral-etal-2023-tackling} & L & 12.6M & 43.6 & 58.5 & \underline{38.9} & 53.9 & \underline{36.2} & 51.7 \\

    VALHALLA~\cite{li2022valhalla} & L & - & 42.7 & 69.3 & 35.1 & 62.8 & 30.7 & 57.5 \\
    CLIP-Trans~\cite{gupta2023cliptrans} & L & - & \underline{43.9} & \underline{70.2} & 37.2 & \underline{65.4} & 34.5 & \underline{61.3} \\
    
    CAP-ALL~\cite{li2021feature} & V + L & - & 39.6 & 57.5 & 33.0 & 52.2 & 27.6 & 46.4 \\
    DCCN~\cite{lin2020dynamic} & V + L & - & 39.7 & 56.8 & 31.0 & 49.9 & 26.7 & 45.7 \\
    Gated Fusion~\cite{wu2021good} & V + L & 2.8M & 42.0 & 67.8 & 33.6 & 61.9 & 29.0 & 56.1 \\
    
    Graph-MMT~\cite{yin2020novel}
    & V + L  & 4.0M &  38.6 & 54.4 &  29.0 &  45.7 &  25.9  &  43.2 \\
  
    VGAMT~\cite{futeral-etal-2023-tackling} & V + L & 13.2M & 43.3 & 58.1  & 38.3 & 53.6  & 35.7 & 51.7 \\
    \hline

    LLAVA-Zeroshot & L & - & 29.5 & 60.6 & 27.0 & 57.3 & 25.1 & 52.3 \\
    LLAVA-LoRA & L & 13.1M & 44.8 & 72.0 & 39.0 & 66.7 & 36.3 & 62.5 \\
    LLAVA-Zeroshot & V + L & - & 30.4 & 61.4 & 26.8 & 57.3 & 25.7 & 52.9 \\
    LLAVA-LoRA & V + L & 13.1M & \textbf{45.0} & \textbf{72.1} & \textbf{39.3} & \textbf{67.3} & \textbf{36.8} & \textbf{63.0} \\
   
    \bottomrule
    
    \end{tabular}
    }
    %\vspace{-.2cm}
    \caption{English (EN) to German (DE) and French (FR) multi-modal translation results in Multi30k dataset. The best scores in each subset are marked \textbf{bold} and the second-best scores are \underline{underlined}.}%\vspace{-.3cm}}
    \label{tab:main_table_fr}
\end{table*}

==> tabs/pbj_recon.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{
    \centering\small
    \begin{tabular}{lcccccccc} \toprule
    \multicolumn{9}{c}{\bf En$\rightarrow$Fr} \\\midrule 
    \bottomrule
    
    \end{tabular}
    }
    %\vspace{-.2cm}
    \caption{Caption}%\vspace{-.3cm}}
    \label{tab:pbj_recon}
\end{table*}
 
